Network Coding with Myopic Adversaries

We consider the problem of reliable communication over a network containing a hidden {\it myopic} adversary who can eavesdrop on some $z_{ro}$ links, jam some $z_{wo}$ links, and do both on some $z_{rw}$ links. We provide the first information-theoretically tight characterization of the optimal rate of communication possible under all possible settings of the tuple $(z_{ro},z_{wo},z_{rw})$ by providing a novel coding scheme/analysis for a subset of parameter regimes. In particular, our vanishing-error schemes bypass the Network Singleton Bound (which requires a zero-error recovery criteria) in a certain parameter regime where the capacity had been heretofore open. As a direct corollary we also obtain the capacity of the corresponding problem where information-theoretic secrecy against eavesdropping is required in addition to reliable communication.

==> adversary_grassmannian.tex <==
    \begin{tikzpicture}
    \newcommand{\asymcloud}[2][.1]{%
\begin{scope}[#2]
\pgftransformscale{#1}%    
\pgfpathmoveto{\pgfpoint{261 pt}{115 pt}} 
  \pgfpathcurveto{\pgfqpoint{70 pt}{107 pt}}
                 {\pgfqpoint{137 pt}{291 pt}}
                 {\pgfqpoint{260 pt}{273 pt}} 
  \pgfpathcurveto{\pgfqpoint{78 pt}{382 pt}}
                 {\pgfqpoint{381 pt}{445 pt}}
                 {\pgfqpoint{412 pt}{410 pt}}
  \pgfpathcurveto{\pgfqpoint{577 pt}{587 pt}}
                 {\pgfqpoint{698 pt}{488 pt}}
                 {\pgfqpoint{685 pt}{366 pt}}
  \pgfpathcurveto{\pgfqpoint{840 pt}{192 pt}}
                 {\pgfqpoint{610 pt}{157 pt}}
                 {\pgfqpoint{610 pt}{157 pt}}
  \pgfpathcurveto{\pgfqpoint{531 pt}{39 pt}}
                 {\pgfqpoint{298 pt}{51 pt}}
                 {\pgfqpoint{261 pt}{115 pt}}
\pgfusepath{fill,stroke}         
\end{scope}}  

\node(root)[circle,radius = 1pt, draw = blue, fill = blue!30]  at (0,0) {};

\node(l1)[below = 0.1 cm of root, color = blue]   {$\vdots$} ;

\node(l22)[below = 0.1 cm of l1, color = blue] {$\dots$} ;

\node(l21)[circle,radius = 1pt, draw = blue, fill = blue!30 , left = 0.05 cm of l22] {} ;

\node(l23)[circle,radius = 1pt, draw = blue, fill = blue!30,  right = 0.05 cm of l22]{} ;

\node(ro) [right = 0.2 cm of l23, color = blue] {$z_{ro}$};

\node(l31) [below = 0.1 cm of l22, color = green!50!black]{$\vdots$};

\node(l32) [left = 0.4 cm of l31, color = green!50!black]{\reflectbox{$\ddots$}};

\node(l33) [right = 0.4 cm of l31, color = green!50!black]{$\ddots$};

\node(l41) [below = 0.1 cm of l31, color = green!50!black]{$\dots$};

\node(l42) [circle,radius = 1pt, draw = green!50!black, fill = green!30, left = 0.6 cm of l41]{};

\node(l43)[circle,radius = 1pt, draw = green!50!black, fill = green!30, right = 0.6 cm of l41]{};

\node(rw) [right = 0.2 cm of l43, color = green!50!black] {$z_{rw}+z_{ro}$};

\node(l51) [below = 0.1 cm of l41, color = red]{$\vdots$};

\node(l52) [left = 0.7 cm of l51, color = red]{\reflectbox{$\ddots$}};

\node(l53) [right = 0.7 cm of l51, color = red]{$\ddots$};

\node(l61) [below = 0.1 cm of l51, color = red] {$\dots$};

\node(l62) [circle,radius = 1pt, draw = red, fill = red!30, right = 0.8 cm of l61]{};

\node(l63) [circle,radius = 1pt, draw = red, fill = red!30, left = 0.8 cm of l61]{};

\node(wo) [ right = 0.2 cm of l62, color = red] {$z_{ro}+z_{rw}+z_{wo}$};

\node(l71) [below = 0.1 cm of l61, color = black] {$\vdots$};

\node(l72) [left = 0.8 cm of l71, color = black] {\reflectbox{$\ddots$}};

\node(l73) [right = 0.8 cm of l71, color = black] {$\ddots$};

\node(l81) [below = 0.1cm of l71, color = black] {$\dots$};

\node(l82) [circle,radius = 1pt, draw = black, fill = black!30!black, right = 1.0 cm of l81]{};

\node(l83) [circle,radius = 1pt, draw = black, fill = black!30!black, left = 1.0 cm of l81]{};

\node(c) [right = 0.2cm of l82] {$\capacity$};

    \end{tikzpicture}

==> grassmannian.tex <==
    \begin{tikzpicture}
    \newcommand{\asymcloud}[2][.1]{%
\begin{scope}[#2]
\pgftransformscale{#1}%    
\pgfpathmoveto{\pgfpoint{261 pt}{115 pt}} 
  \pgfpathcurveto{\pgfqpoint{70 pt}{107 pt}}
                 {\pgfqpoint{137 pt}{291 pt}}
                 {\pgfqpoint{260 pt}{273 pt}} 
  \pgfpathcurveto{\pgfqpoint{78 pt}{382 pt}}
                 {\pgfqpoint{381 pt}{445 pt}}
                 {\pgfqpoint{412 pt}{410 pt}}
  \pgfpathcurveto{\pgfqpoint{577 pt}{587 pt}}
                 {\pgfqpoint{698 pt}{488 pt}}
                 {\pgfqpoint{685 pt}{366 pt}}
  \pgfpathcurveto{\pgfqpoint{840 pt}{192 pt}}
                 {\pgfqpoint{610 pt}{157 pt}}
                 {\pgfqpoint{610 pt}{157 pt}}
  \pgfpathcurveto{\pgfqpoint{531 pt}{39 pt}}
                 {\pgfqpoint{298 pt}{51 pt}}
                 {\pgfqpoint{261 pt}{115 pt}}
\pgfusepath{fill,stroke}         
\end{scope}}  



\node(v1)[circle,radius = 1pt, draw = blue, fill = blue!30 ] at(-0.5,0){} ;

\node(v2)[circle,radius = 1pt, draw = green, fill = green!30] at (0.5,0){} ;

\node(a) [right = 0.2 cm of v2] {$a$};

\node(v3) [circle,radius = 1pt, draw = red, fill = red!30 ] at (0,-1){};

\node(v4) [circle,radius = 1pt, draw = black, fill = black!30 ] at (-1,-1) {};

\node(v5) [circle,radius = 1pt, draw = yellow, fill = yellow!30] at (1,-1) {};

\node(a+1) [right = 0.2 cm of v5] {$a+1$};

%\node(right) [] at (1.25,-0.5) {\reflectbox{$\ddots$}};



\path [->]
(v1)    edge (v3)
        edge (v4)

(v2)    edge (v3)
        edge (v5);
    \end{tikzpicture}

==> uppertail_chernoff.tex <==
\yihan{Do we need the lower tail?}

Here we prove how to get the upper tail Chernoff bound probability $e^{-n^3}$ through the theorem 4.1 in \cite{motwani1995randomized}. The applications of the Chernoff bound are similar in the lemmas' proofs. The main idea is to first get some expected value exponentially small in $n$, then we can apply the upper tail Chernoff bound directly to get our result.

Firstly, by theorem 4.1 in \cite{motwani1995randomized}, for an independent Poisson trails \yihan{Why Poisson trails? Chernoff only requires independent random variables.} with expected value $q^{-\Delta n}$ with some constant $\Delta > 0$, the probability of that the random variable summation to be more than $(1+n^3 q^{\Delta n} )q^{-\Delta n}$ is less than
\begin{align*}
    \left (\frac{e^{n^3 q^{\Delta n}}}{(1+n^3 q^{\Delta n})^{1+n^3 q^{\Delta n}}}\right )^{q^{-\Delta n}}
\end{align*}
Here we consider the case for large $n$ and $q$ so we ignore the constant 1. Thus we have:
\begin{align*}
    \left (\frac{e^{n^3 q^{\Delta n}}}{(n^3 q^{\Delta n})^{n^3 q^{\Delta n}}}\right)^{q^{-\Delta n}} &= \frac{e^{n^3}}{(n^3 q^{\Delta n})^{n^3}}
\end{align*}
Next we compare this term with $e^{-n^3}$.

Since $(\frac{n^3}{e^2})^{-n^3}q^{-\Delta n^4} \leq 1$ for large positive $n$ and $q$, we multiply $e^{-n^3}$ to both sides to get:
\begin{align*}
    e^{n^3} n^{-3n^3} q^{-\Delta n^4} \leq e^{-n^3}
\end{align*}
Note the left part is exactly the direct result of theorem 4.1 in \cite{motwani1995randomized}. Therefore, we proved the upper tail $e^{-n^3}$ in our case.
